Out of Order: How Important Is The Sequential Order of Words in a Sentence in Natural Language Understanding Tasks?

Do state-of-the-art natural language understanding models care about word order - one of the most important characteristics of a sequence? Not always! We found 75% to 90% of the correct predictions of BERT-based classifiers, trained on many GLUE tasks, remain constant after input words are randomly shuffled. Despite BERT embeddings are famously contextual, the contribution of each individual word to downstream tasks is almost unchanged even after the word's context is shuffled. BERT-based models are able to exploit superficial cues (e.g. the sentiment of keywords in sentiment analysis; or the word-wise similarity between sequence-pair inputs in natural language inference) to make correct decisions when tokens are arranged in random orders. Encouraging classifiers to capture word order information improves the performance on most GLUE tasks, SQuAD 2.0 and out-of-samples. Our work suggests that many GLUE tasks are not challenging machines to understand the meaning of a sentence.

==> _ACL2021_arxiv/thang_tables_backup.tex <==
% Thang Note: Unused packages
% \usepackage{times}
% \usepackage{latexsym}
% \usepackage{microtype}
% \usepackage{natbib}
% \usepackage{appendix}
% \usepackage{tikz}
% \usepackage{tikz-dependency}
% \usepackage{qtree}
% \usepackage{amsmath}
% \usepackage{amsfonts}
% \usepackage{graphicx}
% \usepackage{amsthm}
% \usepackage{amssymb}
% \usepackage{url}
% \usepackage[dvipsnames]{xcolor}
% \usepackage[smallerops]{newtxmath}
% \usepackage{subfig}
% \usepackage{multicol}
% \usepackage{tcolorbox}
% \usepackage{adjustbox}
% \renewcommand\colorbox[1]{\adjustbox{margin=3pt {\fboxsep},bgcolor=#1}}

% ----- For this paper 

% \usepackage{soul}
% \sethlcolor{lightgray}

% Add vertical padding within each tabular cell.
% \usepackage[math]{cellspace}
%     \cellspacetoplimit 2pt
%     \cellspacebottomlimit 2pt



% \begin{table}[h]
% \centering\small
% % \setlength\tabcolsep{2pt}
% % \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{lccc}
% \toprule
% & One-time & \multicolumn{2}{c}{Extra-finetuning} \\
% Task & Finetuning & \multicolumn{2}{c}{Improvements} \\
% \cmidrule(l{2pt}r{2pt}){3-4}
% &  & Average & STD \\
% \toprule 
% \texttt{RTE} & 72.2 & \textbf{1.01} & 1.18 \\
% \cmidrule{1-4}
% \texttt{QQP} & 91.12 & \textbf{0.07} & 0.08 \\
% \cmidrule{1-4}
% \texttt{MRPC} & 87.25 & \textbf{0.06} & 1.39 \\
% \cmidrule{1-4}
% \texttt{SST-2} & 94.5 & -0.28 & 0.21 \\
% \cmidrule{1-4}
% \texttt{QNLI} & 92.57 & \textbf{0.14} & 0.24 \\
% \bottomrule
% \end{tabular}
% % }
% \caption{Finetuning evaluation performance on downstream tasks (train and dev sets).}
% \label{tb:second_finetuning}
% \end{table}

% \begin{table}[h]
% \centering\small
% \setlength\tabcolsep{3pt}
% % \resizebox{0.99\textwidth}{!}{
% \begin{tabular}{ccc}
% \toprule
% % \multirow{3}{*}{Task} & \multicolumn{2}{c}{\robertaBase} \\
% % \cmidrule(l{2pt}r{2pt}){2-3}
% \multirow{2}{*}{\robertaBase}& without EF & with EF \\
% & (F1 / Acc) & (F1 / Acc) \\
% \toprule
% SQuAD\_v2 & 80.62 / 80.97 & \textbf{80.75 / 81.09} \\
% \cmidrule(l{2pt}r{2pt}){1-3}
% Adversarial & \multirow{2}{*}{79.04 / 79.04} & \textbf{\multirow{2}{*}{79.73 / 79.73}} \\
% examples only \\
% \bottomrule
% \end{tabular}
% % }

% \caption{Extra-finetuned RoBERTa model is more accurate against adversarial examples.}
% \label{table:extra_finetuning_squadv2}
% \end{table}

% \begin{table}[h]
% \centering\small
% \setlength\tabcolsep{2pt}
% % \resizebox{0.99\textwidth}{!}{
% \begin{tabular}{lcc}
% \toprule
% \cmidrule(l{2pt}r{2pt}){2-3}
% & \multirow{1}{*}{SQuAD\_v2} & No-answer Questions \\
% & (F1 / Acc) & (F1 / Acc) \\
% \toprule
% \robertaBase & 80.62 / 80.97 & 79.04 / 79.04 \\
% \hspace{3mm} + extra finetuning & \textbf{80.75 / 81.09} & \textbf{79.73 / 79.73} \\
% \bottomrule
% \end{tabular}
% % }

% \caption{Extra-finetuned RoBERTa model is more accurate against adversarial examples.}
% \label{table:extra_finetuning_squadv2}
% \end{table}

% \begin{table}[h]
% \centering\small
% \setlength\tabcolsep{2pt}
% % \resizebox{0.99\textwidth}{!}{
% \begin{tabular}{lccc}
% \toprule
% \multirow{1}{*}{Models} & \multicolumn{2}{c}{Tasks (Dev Set)} & \multirow{1}{*}{Type} \\
% \cmidrule(l{2pt}r{2pt}){2-3}
% & \multirow{2}{*}{SQuAD\_v2} & No-answer & \\
% &  & Questions & \\
% & (F1 / Acc) & (F1 / Acc) & \\
% \toprule
% \robertaBase & 80.62 / 80.97 & 79.04 / 79.04 & \multirow{2}{*}{Original} \\
% \hspace{3mm} + extra finetuning & \textbf{80.75 / 81.09} & \textbf{79.73 / 79.73} &  \\
% \cmidrule{1-4}
% \robertaBase & \textbf{66.57 / 66.73} & 80.36 / 80.36 & \multirow{2}{*}{Shuffle} \\
% \hspace{3mm} + extra finetuning & 64.56	64.8 & \textbf{89.05 / 89.05} &  \\
% \bottomrule
% \end{tabular}
% % }

% \caption{Extra-finetuned RoBERTa model is more accurate against adversarial examples.}
% \label{table:extra_finetuning_squadv2}
% \end{table}


% \begin{table}[h]
% \centering\small
% \setlength\tabcolsep{1pt}
% % \resizebox{0.99\textwidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% Task & \multicolumn{5}{c}{Shuffle Dev Set} \\
% \cmidrule(l{2pt}r{2pt}){2-6}
% & RTE & QQP & MRPC & SST-2 & QNLI \\
% & (Acc) & (Acc) & (Acc) & (Acc) & (Acc)  \\
% \toprule
% \robertaBase & 82.56 & 72.2 & 91.12 & 87.25 & 94.5 \\
% \hspace{1mm} + extra finetuning \textbf{(ours)} & 82.56 & 72.2 & 91.12 & 87.25 & 94.5 \\
% \bottomrule
% \end{tabular}
% % }

% \caption{Original performance of 3 base models finetuned on seven GLUE tasks.}
% \label{table:original_performance}
% \end{table}






% \makecell{Q} & \scriptsize
% % \makecell{original \\ text\_a} & \scriptsize
% \colorbox{red!0.619}{\strut How} \colorbox{red!1.6209999999999998}{\strut old} \colorbox{red!0.676}{\strut was} \mybox{red}{ \colorbox{red!0.384}{\strut Tesla}} \colorbox{red!0.9039999999999999}{\strut when} \colorbox{red!0.603}{\strut he} \mybox{blue}{ \colorbox{red!0.91}{\strut became}} \colorbox{red!0.074}{\strut a} \mybox{green}{ \colorbox{red!0.9690000000000001}{\strut citizen}} \colorbox{red!0.47400000000000003}{\strut of} \colorbox{blue!0.188}{\strut the} \colorbox{red!0.843}{\strut US?} & \multirow{3}{*}{99.92} \\
% \cline{1-2}\multirow{2}{*}{A} & \scriptsize \colorbox{blue!1.809}{\strut On} \colorbox{red!8.225}{\strut 30} \colorbox{blue!0.45199999999999996}{\strut July} \colorbox{red!7.341}{\strut 1891,} \colorbox{red!3.3300000000000005}{\strut at} \colorbox{blue!0.013}{\strut the} \colorbox{red!10.101}{\strut age} \colorbox{red!3.9219999999999997}{\strut of} \colorbox{red!15.459999999999999}{\strut 35,} \mybox{red}{ \colorbox{blue!0.991}{\strut Tesla}} \mybox{blue}{ \colorbox{blue!2.311}{\strut became}} \colorbox{blue!1.415}{\strut a} \colorbox{red!1.71}{\strut naturalized} \mybox{green}{ \colorbox{red!2.6270000000000002}{\strut citizen}} \colorbox{red!3.9219999999999997}{\strut of} \colorbox{blue!0.013}{\strut the} \colorbox{blue!1.049}{\strut United} \colorbox{blue!0.02}{\strut States,} \colorbox{red!1.9349999999999998}{\strut and} \colorbox{blue!1.134}{\strut established} \colorbox{blue!0.65}{\strut his} \colorbox{red!0.628}{\strut South} \colorbox{red!0.377}{\strut Fifth} \colorbox{blue!0.636}{\strut Avenue} \colorbox{blue!3.6740000000000004}{\strut laboratory,} \colorbox{red!1.9349999999999998}{\strut and} \colorbox{blue!2.045}{\strut later} \colorbox{blue!1.34}{\strut another} \colorbox{red!3.3300000000000005}{\strut at} \colorbox{red!3.7539999999999996}{\strut 46} \colorbox{red!1.407}{\strut E.} \colorbox{blue!1.246}{\strut Houston} \colorbox{blue!1.6889999999999998}{\strut Street,} \colorbox{red!0.774}{\strut in} \colorbox{red!0.134}{\strut New} \colorbox{blue!1.244}{\strut York.} &  \\
% \hline
% \makecell{Q1} & \scriptsize  \colorbox{blue!2.2030000000000003}{\strut a} \mybox{green}{ \colorbox{red!1.6729999999999998}{\strut Tesla}} \colorbox{red!2.321}{\strut How} \mybox{blue}{ \colorbox{red!5.155}{\strut became}} \colorbox{blue!2.648}{\strut of} \colorbox{red!1.154}{\strut old} \colorbox{red!3.227}{\strut was} \colorbox{blue!2.3970000000000002}{\strut the} \colorbox{red!3.0509999999999997}{\strut he} \colorbox{red!2.732}{\strut when} \mybox{red}{ \colorbox{red!8.205}{\strut citizen}} \colorbox{red!4.046}{\strut US?} & 99.19 \\
% \cline{1-2}\makecell{A} & \scriptsize  \colorbox{blue!2.789}{\strut On} \colorbox{red!5.293}{\strut 30} \colorbox{blue!0.9249999999999999}{\strut July} \colorbox{red!9.908}{\strut 1891,} \colorbox{red!4.313000000000001}{\strut at} \colorbox{blue!0.582}{\strut the} \colorbox{red!11.999}{\strut age} \colorbox{red!1.387}{\strut of} \colorbox{red!20.191}{\strut 35,} \mybox{green}{ \colorbox{red!0.16199999999999998}{\strut Tesla}} \mybox{blue}{ \colorbox{blue!0.959}{\strut became}} \colorbox{red!0.5599999999999999}{\strut a} \colorbox{red!1.196}{\strut naturalized} \mybox{red}{ \colorbox{blue!0.348}{\strut citizen}} \colorbox{red!1.387}{\strut of} \colorbox{blue!0.582}{\strut the} \colorbox{red!0.872}{\strut United} \colorbox{red!0.492}{\strut States,} \colorbox{blue!0.464}{\strut and} \colorbox{red!2.9080000000000004}{\strut established} \colorbox{blue!1.122}{\strut his} \colorbox{blue!2.393}{\strut South} \colorbox{red!2.613}{\strut Fifth} \colorbox{blue!2.186}{\strut Avenue} \colorbox{blue!0.037}{\strut laboratory,} \colorbox{blue!0.464}{\strut and} \colorbox{blue!0.5369999999999999}{\strut later} \colorbox{blue!3.3939999999999997}{\strut another} \colorbox{red!4.313000000000001}{\strut at} \colorbox{red!4.199}{\strut 46} \colorbox{blue!3.029}{\strut E.} \colorbox{red!0.378}{\strut Houston} \colorbox{blue!2.562}{\strut Street,} \colorbox{blue!2.03}{\strut in} \colorbox{blue!0.393}{\strut New} \colorbox{red!1.504}{\strut York.} &  \\
% \hline
% \makecell{Q2} & \scriptsize  \colorbox{red!1.8950000000000002}{\strut when} \mybox{red}{ \colorbox{red!0.35200000000000004}{\strut Tesla}} \colorbox{red!0.749}{\strut was} \colorbox{red!1.127}{\strut he} \mybox{green}{ \colorbox{red!3.012}{\strut citizen}} \mybox{blue}{ \colorbox{red!2.983}{\strut became}} \colorbox{blue!0.993}{\strut the} \colorbox{red!0.989}{\strut a} \colorbox{red!0.296}{\strut of} \colorbox{red!2.791}{\strut US} \colorbox{red!0.662}{\strut How} \colorbox{red!1.353}{\strut old?} & 99.92 \\
% \cline{1-2}\makecell{A} & \scriptsize  \colorbox{blue!2.988}{\strut On} \colorbox{red!6.297}{\strut 30} \colorbox{blue!3.26}{\strut July} \colorbox{red!5.91}{\strut 1891,} \colorbox{red!2.752}{\strut at} \colorbox{blue!3.2779999999999996}{\strut the} \colorbox{red!13.128}{\strut age} \colorbox{red!0.469}{\strut of} \colorbox{red!15.206}{\strut 35,} \mybox{red}{ \colorbox{blue!1.892}{\strut Tesla}} \mybox{blue}{ \colorbox{blue!1.8610000000000002}{\strut became}} \colorbox{blue!0.762}{\strut a} \colorbox{red!0.9560000000000001}{\strut naturalized} \mybox{green}{ \colorbox{red!1.526}{\strut citizen}} \colorbox{red!0.469}{\strut of} \colorbox{blue!3.2779999999999996}{\strut the} \colorbox{red!0.607}{\strut United} \colorbox{red!1.478}{\strut States,} \colorbox{blue!1.9929999999999999}{\strut and} \colorbox{blue!0.501}{\strut established} \colorbox{red!1.121}{\strut his} \colorbox{blue!1.083}{\strut South} \colorbox{blue!0.025}{\strut Fifth} \colorbox{red!2.396}{\strut Avenue} \colorbox{red!2.185}{\strut laboratory,} \colorbox{blue!1.9929999999999999}{\strut and} \colorbox{blue!0.048}{\strut later} \colorbox{blue!1.225}{\strut another} \colorbox{red!2.752}{\strut at} \colorbox{red!4.671}{\strut 46} \colorbox{red!0.047}{\strut E.} \colorbox{red!0.5740000000000001}{\strut Houston} \colorbox{blue!0.724}{\strut Street,} \colorbox{blue!0.8059999999999999}{\strut in} \colorbox{blue!1.4160000000000001}{\strut New} \colorbox{red!0.575}{\strut York.} &  \\
% \hline
% \makecell{Q3} & \scriptsize  \colorbox{red!1.421}{\strut old} \mybox{green}{ \colorbox{red!0.17099999999999999}{\strut Tesla}} \colorbox{red!0.694}{\strut was} \mybox{blue}{ \colorbox{red!3.0429999999999997}{\strut became}} \colorbox{red!1.0739999999999998}{\strut he} \colorbox{blue!0.621}{\strut How} \colorbox{blue!2.574}{\strut the} \mybox{red}{ \colorbox{red!9.525}{\strut citizen}} \colorbox{red!6.152}{\strut when} \colorbox{red!2.137}{\strut of} \colorbox{red!7.988}{\strut US} \colorbox{blue!3.089}{\strut a?} & 99.85 \\
% \cline{1-2}\makecell{A} & \scriptsize  \colorbox{blue!4.717}{\strut On} \colorbox{red!7.928}{\strut 30} \colorbox{blue!2.6100000000000003}{\strut July} \colorbox{red!8.959999999999999}{\strut 1891,} \colorbox{red!1.254}{\strut at} \colorbox{blue!2.835}{\strut the} \colorbox{red!9.616}{\strut age} \colorbox{red!4.234999999999999}{\strut of} \colorbox{red!18.363}{\strut 35,} \mybox{green}{ \colorbox{blue!3.1119999999999997}{\strut Tesla}} \mybox{blue}{ \colorbox{blue!2.019}{\strut became}} \colorbox{red!2.6780000000000004}{\strut a} \colorbox{red!0.29}{\strut naturalized} \mybox{red}{ \colorbox{red!3.4160000000000004}{\strut citizen}} \colorbox{red!4.234999999999999}{\strut of} \colorbox{blue!2.835}{\strut the} \colorbox{blue!0.717}{\strut United} \colorbox{blue!0.32299999999999995}{\strut States,} \colorbox{red!2.771}{\strut and} \colorbox{blue!2.771}{\strut established} \colorbox{blue!0.924}{\strut his} \colorbox{red!0.392}{\strut South} \colorbox{red!1.381}{\strut Fifth} \colorbox{red!1.9709999999999999}{\strut Avenue} \colorbox{blue!0.041}{\strut laboratory,} \colorbox{red!2.771}{\strut and} \colorbox{red!3.511}{\strut later} \colorbox{blue!1.755}{\strut another} \colorbox{red!1.254}{\strut at} \colorbox{blue!0.46299999999999997}{\strut 46} \colorbox{blue!2.427}{\strut E.} \colorbox{blue!0.8210000000000001}{\strut Houston} \colorbox{blue!1.134}{\strut Street,} \colorbox{red!1.168}{\strut in} \colorbox{red!1.551}{\strut New} \colorbox{red!0.079}{\strut York.} &  \\
% \hline
% \makecell{Q4} & \scriptsize  \colorbox{blue!0.368}{\strut of} \mybox{red}{ \colorbox{red!4.977}{\strut citizen}} \colorbox{red!0.116}{\strut was} \colorbox{red!1.746}{\strut How} \colorbox{red!5.651}{\strut old} \colorbox{red!0.008}{\strut the} \colorbox{red!1.7000000000000002}{\strut he} \mybox{blue}{ \colorbox{red!3.6189999999999998}{\strut became}} \colorbox{red!2.895}{\strut when} \mybox{green}{ \colorbox{blue!0.369}{\strut Tesla}} \colorbox{red!2.685}{\strut US} \colorbox{blue!1.0659999999999998}{\strut a?} & 99.86 \\
% \cline{1-2}\makecell{A} & \scriptsize  \colorbox{blue!5.558}{\strut On} \colorbox{red!6.5920000000000005}{\strut 30} \colorbox{blue!2.099}{\strut July} \colorbox{red!8.938}{\strut 1891,} \colorbox{red!4.726}{\strut at} \colorbox{blue!1.486}{\strut the} \colorbox{red!12.431000000000001}{\strut age} \colorbox{red!1.798}{\strut of} \colorbox{red!17.402}{\strut 35,} \mybox{green}{ \colorbox{blue!1.043}{\strut Tesla}} \mybox{blue}{ \colorbox{blue!3.537}{\strut became}} \colorbox{red!1.254}{\strut a} \colorbox{blue!1.3719999999999999}{\strut naturalized} \mybox{red}{ \colorbox{blue!0.451}{\strut citizen}} \colorbox{red!1.798}{\strut of} \colorbox{blue!1.486}{\strut the} \colorbox{red!0.271}{\strut United} \colorbox{red!0.603}{\strut States,} \colorbox{red!2.903}{\strut and} \colorbox{blue!1.6340000000000001}{\strut established} \colorbox{red!1.863}{\strut his} \colorbox{red!1.2109999999999999}{\strut South} \colorbox{red!0.409}{\strut Fifth} \colorbox{blue!2.144}{\strut Avenue} \colorbox{red!0.936}{\strut laboratory,} \colorbox{red!2.903}{\strut and} \colorbox{red!1.298}{\strut later} \colorbox{blue!0.183}{\strut another} \colorbox{red!4.726}{\strut at} \colorbox{red!0.979}{\strut 46} \colorbox{blue!2.099}{\strut E.} \colorbox{blue!2.338}{\strut Houston} \colorbox{blue!1.031}{\strut Street,} \colorbox{blue!1.2349999999999999}{\strut in} \colorbox{red!0.14100000000000001}{\strut New} \colorbox{red!1.237}{\strut York.} &  \\
% \hline
% \makecell{Q5} & \scriptsize   \text{\mybox{green}{ \colorbox{red!6.338000000000001}{\strut citizen}}} \colorbox{red!1.175}{\strut the} \colorbox{blue!0.031}{\strut of} \mybox{blue}{ \colorbox{red!4.707999999999999}{\strut became}} \colorbox{red!4.575}{\strut old} \colorbox{red!1.942}{\strut a} \colorbox{red!0.792}{\strut he} \colorbox{blue!0.48}{\strut was} \colorbox{blue!0.65}{\strut How} \colorbox{red!5.485}{\strut when} \colorbox{red!3.319}{\strut US} \mybox{red}{ \colorbox{blue!2.4989999999999997}{\strut Tesla?}} & 99.71 \\
% \cline{1-2}\makecell{A} & \scriptsize  \colorbox{blue!4.684}{\strut On} \colorbox{red!7.455}{\strut 30} \colorbox{blue!2.725}{\strut July} \colorbox{red!8.054}{\strut 1891,} \colorbox{red!2.666}{\strut at} \colorbox{red!0.43}{\strut the} \colorbox{red!11.455}{\strut age} \colorbox{red!0.692}{\strut of} \colorbox{red!16.909}{\strut 35,} \mybox{red}{ \colorbox{blue!4.285}{\strut Tesla}} \mybox{blue}{ \colorbox{blue!2.9080000000000004}{\strut became}} \colorbox{blue!2.778}{\strut a} \colorbox{blue!1.81}{\strut naturalized} \mybox{green}{ \colorbox{red!0.8670000000000001}{\strut citizen}} \colorbox{red!0.692}{\strut of} \colorbox{red!0.43}{\strut the} \colorbox{red!1.831}{\strut United} \colorbox{red!1.8659999999999999}{\strut States,} \colorbox{blue!0.11}{\strut and} \colorbox{red!0.9860000000000001}{\strut established} \colorbox{blue!0.74}{\strut his} \colorbox{blue!0.924}{\strut South} \colorbox{red!0.066}{\strut Fifth} \colorbox{blue!0.437}{\strut Avenue} \colorbox{red!0.193}{\strut laboratory,} \colorbox{blue!0.11}{\strut and} \colorbox{red!2.015}{\strut later} \colorbox{blue!1.4949999999999999}{\strut another} \colorbox{red!2.666}{\strut at} \colorbox{red!2.911}{\strut 46} \colorbox{blue!1.159}{\strut E.} \colorbox{red!1.459}{\strut Houston} \colorbox{red!0.125}{\strut Street,} \colorbox{red!2.538}{\strut in} \colorbox{blue!0.15}{\strut New} \colorbox{blue!0.292}{\strut York.} &  \\
% \hline

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

